A posteriori error estimates for wave maps into spheres

We provide a posteriori error estimates in the energy norm for temporal semi-discretisations of wave maps into spheres that are based on the angular momentum formulation. Our analysis is based on novel weak-strong stability estimates which we combine with suitable reconstructions of the numerical solution. We present time-adaptive numerical simulations based on the a posteriori error estimators for solutions involving blow-up.

==> CVs/VornameNachname.tex <==
\input{header.tex}
%Bitte nur Änderungen in der Umgebung ShortCV vornehmen.
\begin{ShortCV}{Akademischer Titel Vorname Name}
  \fachgebiet{Besoldungsgruppe}{Stellenbezeichnung}{URL zur Homepage}

  %Bitte die wesentlichen Stationen des wissenschaftlichen Werdeganges ergänzen.
  \werdegang{
  \item[JJJJ] Position/Station/Abschluss und Institution
  \item[JJJJ] Position/Station/Abschluss und Institution
  \item[JJJJ] Position/Station/Abschluss und Institution 
  }
  
  %Für die Publikationsliste bitte eine Datei mit den fünf wichtigsten
  % Publikationen der letzten 5 Jahre als bibtex Eintrag anlegen. 
  % Um Duplikate zu vermeiden bitte diese Datei dem Schema 
  % VornameNachname.bib
  % folgend benennen.
  %Die Datensätze dürfen gern direkt aus ams.org/mathscinet entnommen
  %werden.
  \publikationen{URL zur Publikationsliste}{VornameNachname.bib}

  %Bitte ausgewählte Drittmittelprojekte der letzten Jahre ergänzen
  \drittmittel{\item XXX
  \item XXX
  \item XXX
  }
  % Hier bitte alle weiteren für wichtig erachteten Punkte ergänzen
  % z.B. Editorentätigkeit, Herausgeberschaft, Tagungsorganisation,
  % Preise, ...
  \sonstiges{\item XXX
  \item XXX
  \item XXX
  }
\end{ShortCV}
\input{footer.tex}

==> CVs/footer.tex <==
\end{document}
